MessageGuard: A Browser-based Platform for Usable, Content-Based Encryption Research

This paper describes MessageGuard, a browser-based platform for research into usable content-based encryption. MessageGuard is designed to enable collaboration between security and usability researchers on long-standing research questions in this area. It significantly simplifies the effort required to work in this space and provides a place for research results to be shared, replicated, and compared with minimal confounding factors. MessageGuard provides ubiquitous encryption and secure cryptographic operations, enabling research on any existing web application, with realistic usability studies on a secure platform. We validate MessageGuard's compatibility and performance, and we illustrate its utility with case studies for Gmail and Facebook Chat.

==> background.tex <==
\section{Related Work}
Unger et al.~\cite{unger2015sok} provide a comprehensive overview of end-to-end secure messaging protocols and discuss a variety of key management schemes.
This work demonstrates that there is strong interest in end-to-end encryption within the security community.
Unfortunately, examining the systems highlighted by the survey makes it clear that few proposals have ever undergone user studies, making it unclear if these proposals are actually helpful to end users.
This is especially troubling, as previous work has shown a disconnect between what security experts consider to be a good system and what users consider to be usable~\cite{whitten1999why,dhamija2005battle,ruoti2015authentication}.
This highlights the need for engagement by the HCI community in end-to-end encryption research.

One area of end-to-end encryption that has received some level of attention from HCI researchers is secure email.
Whitten and Tygar~\cite{whitten1999why} conducted the first formal user study of a secure email system (i.e., PGP 5).
They found serious usability issues with key management and users' understanding of the underlying public key cryptography. 
More recent studies have also found that even after more than a decade and a half, the security community has still failed to make PGP usable by average users~\cite{sheng2006why,ruoti2015why}.

Still, there has been some progress towards usable, secure email.
A study by Garfinkel et al.~\cite{garfinkel2005johnny} showed that automatic key management significantly increased the usability of secure email.
Using automatic encryption, Atwater et al.~\cite{atwater2015leading} where able to significantly improve the usability of Mailvelope, a PGP-based secure email tool.\footnote{We note that Atwater et al.'s system does not include several practical key management steps that users would be required to perform, limiting the applicability of their results. With \mg, it would be possible to rapidly prototype Atwater et al.'s proposed modification to PGP, but with full key management, allowing for a more accurate evaluation of their ideas.}
Finally, using \mg we have built [Redacted], which has been shown to be highly successful at helping users correctly send encrypted email and consistently outperforms other secure email systems~\cite{ruoti2013confused,ruoti2016private,ruoti2016we}.

%NOTE: Is there anything else we need to mention here. We discuss other technologies briefly in goals section, and in depth in our comparison that is no longer included...


==> intro-orig.tex <==
\section{Introduction}

Users share private information on the web through a variety of applications, such as email, instant messaging, social media, and document sharing.
HTTPS protects this information during transmission, but does not protect users' data while at rest.
Additionally, middleboxes can weaken HTTPS connections by failing to properly implement TLS or adequately validate certificate chains~\cite{liang2014https}.
Even if a website correctly employs HTTPS and encrypts user data while at rest, the user's data is still vulnerable in a number of ways --- honest-but-curious websites that mine user data~\cite{ruoti2013confused}, misbehaving third-party libraries~\cite{stefan2014protecting}, compromise of the website's back end, poor protocol design and implementation~\cite{foster2015security,durumeric2015neither,holz2016tls}, and coerced information disclosure by governments.

This state of affairs motivates the need for {\em content-based} encryption of user data.
%, rather than relying on the connection-based encryption afforded by protocols like HTTPS.
In content-based encryption, users' sensitive data is encrypted at their own computer and only decrypted once it reaches the intended recipient, remaining opaque to the websites that store or transmit this encrypted data.
The best known examples of content-based encryption are secure email (e.g., PGP, S/MIME) and secure instant messaging (e.g., OTR).
In addition to protecting communication, content-based encryption can protect any data users store or distribute online; for example, files stored in the cloud (e.g., DropBox, Google Drive) or tasks in a web-based to-do list.

To address the need for content-based encryption, we have developed \mg, a system that retrofits existing web applications with content-based encryption.
\mg uses security overlays~\cite{ruoti2013confused} to isolate a user's sensitive content from web applications, ensuring that only an encrypted copy of the user's data is available to those web applications.
The contributions of MessageGuard include:

\begin{enumerate}

\item
\mg is the first content-based encryption system that is designed to work with all websites, in all browsers, and all platforms (desktop and mobile).
Additionally, \mg is able to independently secure web applications, without requiring their cooperation, allowing it to scale with the ever-increasing number of applications on the web.

\item
In addition to the generic \mg interfaces that support most web applications, \mg supports customized per-application interfaces.
These interfaces can be used to increase \mg's usability for the most widely used applications (e.g., Webmail, Facebook) and to  interoperate with existing content-based encryption systems (e.g., PGP, S/MIME).
We have built custom interfaces for Gmail and Facebook Chat.

\item
We have validated \mg's compatibility, performance, and usability.
We show that \mg supports all of the Alexa Top 50 websites with little impact on page load times.
Additionally, results from seven usability studies (involving a total of 220 participants) demonstrate that users find \mg's  custom interfaces to be highly usable, with SUS (System Usability Scale~\cite{brooke1996sus}) scores ranging between 70 -- 80.

\end{enumerate}

\subsection{\mg As a Platform}

During the development of \mg, we noticed several things:
First, there are many open HCI and security questions regarding content-based encryption~\cite{garfinkel2014usable}.
Second, far too few ideas for content-based encryption are tested empirically, even though previous research has shown that many issues are only discovered during user testing~\cite{whitten1999why,ruoti2015authentication,ruoti2016we}.
Thus, participating in usable, content-based encryption research is a costly affair, requiring researchers to either build a system from scratch~\cite{fahl2012confidentiality,he2014shadowcrypt} or to make substantial modifications to one of the existing open source tools~\cite{atwater2015leading}.\footnote{Substantial modifications are needed because existing open source content-based encryption tools are unusable~\cite{ruoti2015why}.}
To address these concerns, we improved the modular design of \mg so that it could effectively serve as a platform for HCI and security research of content-based encryption.
As a platform, \mg has several key benefits:

\begin{enumerate}

\item
{\em Accelerate the creation of content-based encryption prototypes.}
\mg provides a fully working content-based encryption system, including user interfaces, messaging protocols, and key management schemes.
The design of \mg allows researchers to easily modify only the portions of the system they wish to experiment with, while the remaining portions continue operating as intended.
This simplifies development and allows researchers to focus on their areas of expertise.

For example, HCI researchers can focus on researching user interface design, while allowing \mg to handle the security of overlays and the underlying cryptography.
While HCI researchers could alternatively create mock-systems that do not actually secure content, this runs the risk of creating interfaces that have no way to be realized in an actual secure system, rendering the research invalid.

\item
{\em Enables security researchers to test the usability implications of their proposals.}
While their is a large body of work on messaging protocols and key management schemes for content-based encryption~\cite{unger2015sok}, too little of it has been subjected to formal usability evaluation.\footnote{
This is problematic as experience has shown that many proposals with strong theoretical foundations are either unfeasible in real-world situations~\cite{garrison2016practicality} or have problems that are only apparent when studied empirically~\cite{whitten1999why,dhamija2005battle,ruoti2015authentication}
}
With \mg, security researchers can leverage the existing user interfaces to provide usable prototypes. 
When new interface elements are required, they can collaborate with usability experts to conduct usability evaluations of their proposals.

\item
{\em Simplifies the comparison of competing ideas.}
\mg can be used to rapidly develop prototypes for use in A/B testing~\cite{ruoti2016private}.
Two prototypes built using \mg will only differ in the areas that have been modified by researchers.
This helps limit the confounding factors that have proven problamatic in past comparison of content-based encryption systems~\cite{ruoti2013confused,atwater2015leading,ruoti2016we}.
The usability studies reported in this paper provide a baseline for comparison against future work built on \mg.

\item
{\em Provides a platform for sharing research results.}
Researchers who create prototypes using \mg can share their specialized interfaces, protocols, or key management schemes as one or more patches,\footnote{A diff-based patch of \mg's code base.}, allowing other researchers to leverage and replicate their work.
Additionally, successful research that would benefit all \mg prototypes can be merged into \mg's code base, allowing the community to benefit from these advances and reducing fragmentation of efforts.%\footnote{This is similar to the benefit that LLVM has provided to the compiler research community.}

\end{enumerate}

%While there has been significant research into content-based encryption~\cite{garfinkel2014usable,unger2015sok} (predominantly in the areas of secure email and instant messaging), this work has largely been limited to security researchers.
%Still, a significant portion of this work is theoretical, and most of the systems that have been implemented and tested have abysmal usability~\cite{whitten1999why,sheng2006why,ruoti2013confused,atwater2015leading,ruoti2015why,ruoti2016we}.
%As such, two things are clear: first, security researchers need a method for implementing and testing their proposed solutions and second, the field of content-based encryption needs greater participation from the HCI community.

\subsection{Areas of Potential Research}
%% discuss comparative research as well! E.g. A/B testing

%% discuss what this platform enables in HCI research
%% - key management (especially managing your own keys, portability, etc)
%% - authentication (is this really Scott Ruoti?)
%% - comparative research

MessageGuard is designed to be a platform for security and usability researchers 
to cooperate and leverage each other's work in ways that could accelerate the 
development and understanding of usable, secure content-based encryption.

Security researchers can add new protocols, algorithms, and mechanisms into \mg and immediately leverage
proven usability features. 
If the additions can be transparently integrated, the resulting prototype serves as a proof-of-concept 
that the design is seamless and introduces no new usability issues. 
It can also provide a real-world environment for performance testing.
Some examples of potential research includes certificate revocation, certificate transparency, 
CONIKS, additional authentication factors, biometrics, single sign-on, smartphone assisted key discovery, hardware tokens,
and helping users transition to stronger forms of key management. 
Usability researchers can assist in developing usable modifications to support the new security mechanisms and conducting user studies. 
Some potential areas include warning messages, notifications, 
tutorials, icons, and settings.
Other open questions to explore include how to create spoof-proof front-end interfaces, how to authenticate other users before engaging in a secure interaction, and how migrate encryption keys to new devices. 
The results can be compared to prior results with \mg. 

Usability researchers can incorporate new usability features onto existing content-based encryption 
approaches such as PGP, S/MIME, IBE, ABE.
This can facilitate proper A/B testing of proposed usability components, such new encryption metaphors,
warning messages, notifications, tutorials, new color schemes, manual key management, polymorphic warnings,
and authenticating a public key.

The MessageGuard platform has the potential to fundamentally change our ability to do comparative research in 
usable security. 

\subsection{Roadmap}
In \S2 we describe Related Work. In \S3 we give the threat model and design of ubiquitous, content-based encryption for the web. In \S4 we detail the design and implementation of \mg. In \S5 we describe how \mg can be used as a platform for HCI and security research into content-based encryption on the web, including two case studies where we used \mg to build research prototypes.
In \S6 we present our validation of \mg and we conclude this paper in \S7.

